Non-Functional Requirements for Machine Learning: An Exploration of System Scope and Interest

Systems that rely on Machine Learning (ML systems) have differing demands on system quality compared to traditional systems. Such quality demands, known as non-functional requirements (NFRs), may differ in their definition, scope, and importance from NFRs for traditional systems. Despite the importance of NFRs for ML systems, our understanding of their definitions and scope -- and of the extent of existing research in each NFR -- is lacking compared to our understanding in traditional domains. Building on an investigation into importance and treatment of ML system NFRs in industry, we make three contributions towards narrowing this gap: (1) we present clusters of ML system NFRs based on shared characteristics, (2) we use Scopus search results -- as well as inter-coder reliability on a sample of NFRs -- to estimate the number of relevant studies on a subset of the NFRs, and (3), we use our initial reading of titles and abstracts in each sample to define the scope of NFRs over parts of the system (e.g., training data, ML model, or other system elements). These initial findings form the groundwork for future research in this emerging domain.

==> Discussion.tex <==
%In this section, we discuss our study findings. We organize this discussion by RQ. 

%Things to discuss here:

%\begin{itemize}
%\item[RQ1] Can the set of ML system NFRs be grouped into a small number of clusters based on shared characteristics??
%  \item[RQ2] Which NFRs have received the most, or least, attention in existing research literature?
%  \item[RQ3] Over which part of the ML system can each NFR be defined?
%\end{itemize}


\smallskip\noindent\textbf{NFR Clustering (RQ1):}  Previous work has presented NFRs in terms of a hierarchy (e.g.,~\cite{cavano1978framework}) or as part of a interdependency graph (e.g.,~\cite{chung2012non}). Our goal was not to suggest a definite hierarchy, but to group NFRs to clarify relatedness and scope, particularly for future research studies. For example, a study may focus on a particular cluster or one or two related NFRs. These clusters can also help practitioners  understand the similarity of NFRs and provide guidance on which related NFRs they should consider while developing ML systems.


\smallskip\noindent\textbf{Estimated Number of Publications (RQ2):} We can reflect on the number of papers found via Scopus search, or predicted via our ICR results.
The number of papers found for  accuracy is very high as one would predict, as  researchers and  practitioners are focusing mainly on the accuracy of ML systems. We were surprised that no publication was found for  retrainability even though practitioners in~\cite{habibullah2021non} mentioned retrainability is an important NFR for ML systems. Retrainability is a NFR which is exclusively ML-specific, perhaps these ideas are being discussed using terms which are less recognizable as an NFR.  Similarly, we were surprised by so few search results on testability, but this may again be due to a different use of terms, perhaps researchers are using test or testing.  We expected more search results on fairness as we perceive that researchers and practitioners are currently focusing on this topic. This may be due to the commonality and split of results amongst bias, fairness, and ethics.  We found more papers for usability than we expected, even excluding for those papers using usability as applicability, but find it encouraging that research is focusing on these human-oriented aspects.  

From the clustering point of view, we have listed the sum of raw search results per cluster.  Although this is only an initial rough estimate of interest, we can see a particular interest in cluster 4, including performance.  In ML terminology, we note that performance is often used to denote a form of accuracy, how correct the results are, as opposed to capturing running time or memory measures as the term is often used in typical SE.  We note that the performance and accuracy clusters (4 and 1) show the most raw results, followed by the security cluster.  These results are generally in line with our expectations.  We find that cluster 7 containing those NFRs which are hard to cluster actually has a relatively large number of raw results, mainly due to the inclusion of complexity.  We are particularly surprised that clusters 2 containing explainability and cluster 4 containing bias show relatively less raw results.  It seems that even though these are perceived as hot topics in ML research, either the volume of papers is still relatively small, or this work includes terms which differ from the NFRs included as part of our search. 

While going through the 50 titles and abstracts, we found that for some NFRs it was difficult to determine inclusion/exclusion, as is shown by our poor ICR results.  For example, we had particularly low results for ethics and explainability, even though these are often perceived as popular topics in ML research.  This popularity may have contributed to our difficulties.  In other cases, we can often make a clear distinction between NFRs over parts of the ML system and using ML to improve an NFR in another system, e.g., traceability of ML solutions vs. the many papers using ML to find trace links.  With topics like ethics and explaininability, the focus of most papers was on the ML systems themselves, i.e., many papers were relevant.  In these cases, future work may have to work harder on providing clear definitions or specific criteria.  

%Talk about which clusters were ranked highest/lowest, do we see a theme here. Could give the sum/cluster?

%which NFRs are surprising to be ranked so high or so low, and why?

%Surprised so few on testability, maybe not using this term?  Testing?  

\smallskip\noindent\textbf{NFR Scoping Over System Elements (RQ3):} When looking for trends or patterns in our preliminary determination of NFR scope, we can see that most NFRs can be defined over the whole system because the whole system is similar to the scope of NFRs over traditional systems. We see that all NFRs apply over the whole system, and almost all apply over the model, and most to the algorithm. On the other hand, fewer NFRs can apply to the training data and the results, but there is no clear pattern here. We do not find that NFRs always can be applied to the results and data together, sometimes it is one or the other or both.  We intend to continue this work towards a framework to guide NFR exploration, consideration and measurement over ML systems.  We hope that such exploration can lead to a deeper understanding of what makes NFRs applicable to different system parts, and why.

Note that our estimation of NFR scope over system parts as indicated in Table~\ref{tab:nfrdefinedover} is a first pass based on our experiences and on covering the selected abstracts. The scope of NFRs can and likely will evolve over time as more data an experience is gathered, particularly as we and others find more examples, and especially metrics, for NFRs over different parts of an ML system.

%Any trends in the results?   Most NFRs can be defined over the whole system because the whole system is similar scope to traditional NFRs, makes sense to talk about NFRs over a system.

%Work towards a framework to guide NFR exploration, consideration and measurement over NFR systems, part of larger research agenda.  

==> Methodology.tex <==
Though NFRs for traditional software are fairly well-explored, there is still gaps in foundation of knowledge on NFRs for ML systems. We are eager to learn which NFRs for ML systems have been explored by other researchers and which are yet to investigate. We also want to learn how %others have defined, identified and measured  NFRs for ML-enabled systems and which challenges they experienced.
NFRs for ML are perceived by other researchers in different computer science applications. 

Hence, our study has been undertaken as a Systematic Literature Review (SLR) as the research aimed at identifying, and reporting the overview of the current state-of-the-art of NFRs for ML in research. 
%defining and measuring non-functional requirements (NFRs), and their challenges in ML-enabled systems.
The common reason for undertaking an SLR is to get a fair, unbiased, and credible evaluation and summary of existing evidence concerning a technology or a research topic ~\cite{kitchenham2007guidelines}. Therefore, an SLR is an appropriate method for our research, as SLR is an appropriate method for identifying, assessing, analyzing, evaluating, and interpreting published relevant literature in order to investigate a specific research question or phenomenon~\cite{kitchenham2007guidelines}.

To perform systematic literature review we adopted the guidelines proposed by Kitchenham et al.~\cite{kitchenham2007guidelines}, and adopted the systematic inclusion of references defined by Wohlin \cite{wohlin2014guidelines}. To outline our systematic literature review process in a clear and transparent manner, a review protocol should be developed. The development of a review protocol must ensure rigor and repeatability. To ensure the quality, and reduce researchers' bias during review process, we adopted the review protocol proposed in \cite{ali2010systematic}. In particular, the review protocol defines the research questions (Section~\ref{sec:researchquestions}), search strategy (Section~\ref{sec:searchstrategy}) to identify the relevant literature, inclusion and exclusion criteria (Section~\ref{sec:criteria}) to filter relevant studies, and methodology to extract (Section~\ref{sec:dataextraction}) and synthesize (Section~\ref{sec:synthesis}) retrieved information in order to address the research questions. The review protocol was developed following the process presented in Fig.~\ref{fig:Review_protocol_development_process}

\begin{figure} 
How Interested are Researchers in Non-Functional Requirements
for Machine Learning?
Khan Mohammad Habibullah
Gregory Gay
Jennifer Horkoff{khan.mohammad.habibullah,jennifer.horkoff }@gu.se
greg@greggay.com
Chalmers | University of Gothenburg
Gothenburg, Sweden
ABSTRACT
To be added
CCS CONCEPTS
•Software and its engineering →Extra-functional proper-
ties; Requirements analysis; •Computing methodologies →
Machine learning.
KEYWORDS
Non-Functional Requirements, Machine Learning, Machine Learn-
ing System, Bibliometrics
ACM Reference Format:
Khan Mohammad Habibullah, Gregory Gay, and Jennifer Horkoff. 2022.
How Interested are Researchers in Non-Functional Requirements for Ma-
chine Learning?. In CAIN ’22: 1st International Conference on AI Engineer-
ing, May 21–22, 2022, Pittsburgh, PA. ACM, New York, NY, USA, 9 pages.
https://doi.org/10.1145/1122445.1122456
1 INTRODUCTION
Machine Learning (ML), a rapidly developing branch of Artificial
Intelligence (AI), has gained much attention in recent years, and
is increasingly used in decision making and prediction applica-
tions that influence every aspect of our lives. ML-enabled systems
are increasing companies’ capabilities for accelerating and improv-
ing their innovation; and software intensive-industries, such as
Facebook [32], are employing ML-techniques to develop different
intelligent applications.
ML systems are enabled by algorithms that use large amounts
of data for the learning process, and automatically performing
decision-making and predicting tasks that are challenging to achieve
via traditional software [41]. The success stories of ML-enabled
systems include image recognition, natural language processing,
Permission to make digital or hard copies of all or part of this work for personal or
classroom use is granted without fee provided that copies are not made or distributed
for profit or commercial advantage and that copies bear this notice and the full citation
on the first page. Copyrights for components of this work owned by others than ACM
must be honored. Abstracting with credit is permitted. To copy otherwise, or republish,
to post on servers or to redistribute to lists, requires prior specific permission and/or a
fee. Request permissions from permissions@acm.org.
CAIN ’22, May 21–22, 2022, Pittsburgh, PA
©2022 Association for Computing Machinery.
ACM ISBN 978-1-4503-XXXX-X/18/06. . . $15.00
https://doi.org/10.1145/1122445.1122456
complex games, and estimating insurance [29, 41]. The applica-
tion areas of ML are quite vast and range from quality of edu-
cation [10, 24] and healthcare [19, 20]; recommender system in
social [3, 11, 33, 39], and e-commerce [34]; and enforcing the law
and policing [14, 17, 31, 35, 42] services to highly safety-critical and
regulated products, such as autonomous vehicle industry.
ML-enable systems combine high computational power (espe-
cially GPUs), a large amount of data, and complex algorithms that
make the system more complex and vulnerable as exhaustive test-
ing is time-consuming and expensive. Another fundamental chal-
lenge for developing and deploying ML-enabled systems is the
components of ML do not behave in the predefined conventional
manner [25]. Furthermore, describing non-functional requirements
(NFRs) and ensuring the fulfillment of these requirements for such
ML-enabled complex systems become more difficult and threaten
the system’s development. Therefore, despite the advances allowed
by ML, much recent attention has been paid to certain qualities of
ML solutions, particularly on fairness [28], transparency [8], pri-
vacy [9], security [36], safety [13]. From a Requirement Engineering
(RE) perspective, such qualities are also known as non-functional
requirements (NFRs) [15]. According to Glinz, “NFR is an attribute
or a constraint on a system”, where attributes are performance or
quality requirements [21].
NFRs have been part of software engineering for many years,
and research has focused on effectively dealing with NFRs for more
than 40 years e.g., [12]. Although much work has been devoted
to NFRs, dealing with NFRs is still challenging in modern systems
development [27]. Studies demonstrate that NFRs are inherently
difficult and challenging to express explicitly [18], and even more
difficult to verify or validate [37]. The identification, definition, and
measurement of NFRs for a system becomes more critical when ML
comes into play [22, 25].
Much of our accumulated knowledge concerning NFRs may be
no longer applicable when dealing with ML-enabled systems. Some
NFRs, such as fairness, explainability, become more prominent;
accuracy, privacy, become relevant; and usability, interoperability,
become less important [22, 28, 38]. Furthermore, yet unexplored
NFRs, such as retrainability, may become important for ML-enabled
systems. Moreover, the meaning and interpretation of NFRs may
differ and may often not be well understood [7].
Researchers have started working on the identification, defini-
tion, and measurement of NFRs; and finding and resolving existing
challenges related to NFRs for ML-enabled systems. Empirical re-
search has been done to identify how SE knowledge can be applied
CAIN ’22, May 21–22, 2022, Pittsburgh, PA Habibullah et al.
In the future work of [22], the authors intended to conduct a
survey to validate and refine the findings of interview study with
more participants. They also mentioned to work on a systematic
literature review for NFRs in ML based systems, that will allow to
more precisely compare the focus of the industry to the focus of
the literature.
2.4 Our Attempt to Conduct an SLR on NFRs for
ML
We got the inspiration from the future work of [22], and primarily
considered the NFRs identified from the interview study to perform
a systematic literature review. At first, we defined all NFRs listed in
Table 1 to understand the meaning of the NFRs and to identify the
NFRs with similar meaning. Then we have created different clusters
of NFRs, putting similar and related NFRs in the same cluster, shown
in 2. It is not possible to accommodate all NFRs in a single SLR,
as the research space is very big and there are many published
research papers for each NFR for ML. Therefore, we decided to
include the cluster in our SLR study where less research has been
done compared to other clusters.
3 METHODOLOGY
Though NFRs for traditional software are fairly well-explored, there
is still gaps in foundation of knowledge on NFRs for ML-enabled
systems. We are eager to learn Which NFRs for ML-enabled systems
have been explored by other researchers and which are yet to
investigate. We also want to learn how NFRs for ML are perceived
by other researchers in different computer science applications.
Hence, our study has been undertaken as a Systematic Literature
Review (SLR) as the research aimed at identifying, and reporting the
overview of the current state-of-the-art of NFRs for ML in research.
The common reason for undertaking an SLR is to get a fair, unbi-
ased, and credible evaluation and summary of existing evidence
concerning a technology or a research topic [30]. Therefore, an SLR
is an appropriate method for our research, as SLR is an appropri-
ate method for identifying, assessing, analyzing, evaluating, and
interpreting published relevant literature in order to investigate a
specific research question or phenomenon [30].
To perform systematic literature review we adopted the guide-
lines proposed by Kitchenham et al. [30], and adopted the system-
atic inclusion of references defined by Wohlin [44]. To outline our
systematic literature review process in a clear and transparent man-
ner, a review protocol should be developed. The development of
a review protocol must ensure rigor and repeatability. To ensure
the quality, and reduce researchers’ bias during review process,
we adopted the review protocol proposed in [2]. In particular, the
review protocol defines the research questions (Section 3.1), search
strategy (Section ??) to identify the relevant literature, inclusion
and exclusion criteria (Section 3.4) to filter relevant studies, and
methodology to extract (Section ??) and synthesize (Section ??)
retrieved information in order to address the research questions.
The review protocol was developed following the process presented
in Fig. 3
3.1 Research Questions
There is lack of knowledge on NFRs for ML-enabled systems, and
the perception and current treatment of NFRs have yet to be ex-
plored. Hence, our goal in this research is to explore NFRs for
ML-systems and get an idea of the ceiling level of publications for
each NFR, to cluster NFRs based on common themes, to identify
the NFRs that do not belong to a cohesive cluster, and to identify
NFRs which got less attention to the researchers.
We refined the research goals to the following research questions:
RQ1 How can we cluster NFRs based on common themes, which
are relevant for ML?
RQ2 Which NFRs are emphasized in more or less in ML literature?
RQ3 In which part of the ML-system the NFRs are defined?
3.2 Clustering
For creating clusters of NFRs, we primarily considered the NFRs
listed as important for ML-systems in the interview study [22].
All the NFRs were defined with general definitions based on our
experience and with the help of formal definitions to understand the
meaning of those NFRs and identify the NFRs with similar purposes.
Then we created different clusters of NFRs, putting related NFRs
with similar meanings in the same cluster. We also created a separate
cluster for those NFRs with different meanings and could not be
put into any of the clusters of NFRs with similar purposes.
3.3 Publication Volume Estimation
3.3.1 Initial Paper Search. Search Scope
The scope of our search is limited in two dimensions: time (publi-
cation time period) and space (publication venues). In terms of time,
we selected the papers published until September 2021. In terms of
space, a database search was made to identify the research papers
which should be included in the SLR. The selection of databases
and resources to search for relevant literature is very important in
an SLR. We used automatic search as a search method to identify
the related studies for our systematic literature review. Automatic
search refers to the searching technique performed by executing
search strings on search engine of electronic data sources or elec-
tronic databases. The databases’ selection was based on the avail-
ability of a large amount of related scientific papers, i.e., journal
articles, books, and conference proceedings. We selected Scopus (
https://www.scopus.com ), a meta-database for searching related
research papers, which includes research papers from reputed peer-
reviewed journals; conferences; and digital databases, such as IEEE
Xplore digital library ( http://ieeexplore.ieee.org ), ACM digital li-
brary ( https://dl.acm.org ), Elsevier (https://www.elsevier.com/).
The selected source is considered one of the most representative
and rich in content for Software Engineering research and is used
in many other SLRs [? ]. Editorials, abstracts, book chapters, work-
shops, poster sessions, prefaces, article summaries, interviews,
news, reviews, comments, news, reviews, tutorials, panels, and
discussions were excluded from the search.
Search Terms Identification and Search String Development
The strategies applied to construct the search string are described
as follows:
How Interested are Researchers in Non-Functional Requirements for Machine Learning? CAIN ’22, May 21–22, 2022, Pittsburgh, PAInterpretability Transparency Explainability
Justifiability
Accuracy Reliability Reproducibility
Integrity Correctness Fault 
tolerance
NFRs for ML Performance Efficiency ScalabilityBias Fairness
Domain 
adaptation Flexibility Adaptability
Interoperability Portability Reusability
Security Safety
Privacy Trust
Repeatability
Ethics
Consistency
Usability Completeness Maintainability
Traceability Testability Retrainability
Figure 2: NFRs Clusters
At first we derived the major terms (e.g., machine learning, non-
functional requirements etc.) focusing on identification of non-
functional requirements for ML in computer science area. Then
we identified alternative synonyms and/or spelling for the major
terms from the keywords of related literature, and from the discus-
sion of the authors of this paper. We also split major terms into
more specific and clear terms. For example, we split general term
non-functional requirements for ML-enabled systems as reliability,
usability, explainability, efficiency etc., which we found from [22],
described in 2. At last we used boolean operators for conjugation,
i.e., AND for concatenation of major terms and OR operator to
concatenate the alternative synonyms and spelling.
The search terms are built based on the identified population,
intervention, and outcome.
Population: Non-functional requirements and their challenges
identification process
Intervention: Current research and practices in the industry
Outcomes: Understanding non-functional requirements and their
challenges in machine learning context.
The alternative synonyms and spelling for major terms identified
are:
• Machine learning: (“machine learning" OR “supervised
learning" OR “unsupervised learning" OR “reinforcement
learning" OR “deep learning")
• Non-functional requirements: (“repeatability” OR “relia-
bility” OR "accuracy" OR “reproducibility” OR “consistency”
OR “integrity” OR “correctness” OR “fault tolerance” OR
“interpretability” OR “transparency” OR “explainability” OR
“justifiability” OR “ethics” OR “bias” OR “fairness” OR “perfor-
mance” OR “efficiency” OR “scalability” OR “domain adapta-
tion” OR “flexibility” OR “adaptability” OR “interoperability”
OR “portability” OR “reusability” OR “security” OR “trust”
OR “safety” OR “privacy” OR “usability” OR “completeness”
OR “maintainability” OR “traceability” OR “testability” OR
“retrainability”)
We have searched literature in the database for all the non-
functional requirements mentioned in 2 using the search string.
The following example search terms are used to identify related
research papers from database for specified NFRs:
To identify papers on interoperability of ML-ebabled systems
we have used

    \centering
      \includegraphics[width=.5\textwidth]{review_protocol_development_process.pdf}
    \vspace{-0.6cm}
    \caption{Review protocol development process.}
    \label{fig:Review_protocol_development_process}
    \vspace{-0.5cm}
\end{figure}


\subsection{Research Questions}\label{sec:researchquestions}

There is lack of knowledge on NFRs for ML-enabled systems, and the perception and current treatment of NFRs have yet to be explored. Hence, the centeral research question is: 

\begin{itemize}
    \item[RQ1.] What is the perception and current treatment of NFRs in ML in academic and grey literature?
\end{itemize}

Note: define grey literature.  

We refine this RQ1 into more detail as follows:

\begin{itemize}
How can we cluster NFRs which are relevant for ML?
  \item[RQ1.1.]  Which NFRs are emphasized in more or less in ML literature?
  which part of the ML-system the NFR are defined?
  
  \item[RQ1.2.]  what domains are addressed by the literature?
  \item[RQ1.3.]  What domain-specific problems are addressed by the literature?
  \item[RQ1.4.]  What NFR and ML-related challenges or limitations are perceived?
  \item[RQ1.5.]  How are NFRs related to ML currently defined and measured?
  \item[RQ1.6.]  Over what aspects of the system are NFRs defined and measured?
  \item[RQ1.7.]  What measurement-related challenges for NFRs in an ML-context exist?
  \item[RQ1.8.]  Does the ML literature consider trade-offs among NFRs? If so, which trade-offs?
  
 \item[RQ1.9.] Are there any trends or differences on the treatments of NFRs depending on the problem addressed, ML approach or domain (e.g., healthcare, automotive)? 
 
  \item[RQ1.10.] Are there any trends or differences on the treatments of NFRs depending on context (e.g., details of the specific case)? 
\end{itemize}

\subsection{Search Scope} \label{sec:searchscope} 

The scope of our search is limited in two dimensions: time (publication time period) and space (publication venues). 
%and quality ( quality of the identified papers). 
In terms of time, we selected the papers published until September 2021.
%, because, we started sorting the retrieved papers after September 2021.Any paper published after September 2021 is not included. 
% In terms of space, we selected the papers which are indexed by Scopus (https://www.scopus.com/), and published in peer-reviewed journal, conference, or workshop. 
In terms of space, a database search was made to identify the research papers which should be included in the SLR. The selection of databases and resources to search for relevant literature is very important in an SLR. We used automatic search as a search method to identify the related studies for our systematic literature review. Automatic search refers to the searching technique performed by executing search strings on search engine of electronic data sources or electronic databases. The databases' selection was based on the availability of a large amount of related scientific papers, i.e., journal articles, books, and conference proceedings. We selected Scopus ( https://www.scopus.com ), a meta-database for searching related research papers, which includes research papers from reputed peer-reviewed journals; conferences; and digital databases, such as IEEE Xplore digital library ( http://ieeexplore.ieee.org ), ACM digital library ( https://dl.acm.org ), Elsevier (https://www.elsevier.com/).
The selected source is considered one of the most representative and rich in content for Software Engineering research and is used in many other SLRs~\cite{keele2007guidelines}. Editorials, abstracts, book chapters, workshops, poster sessions, prefaces, article summaries, interviews, news, reviews, comments, news, reviews, tutorials, panels, and discussions were excluded from the search.

\subsection{Search Terms Identification and Search String Development} \label{sec:searchterms}

The strategies applied to construct the search string are described as follows:

At first we derived the major terms (e.g., machine learning, non-functional requirements etc.) focusing on identification of non-functional requirements for ML in computer science area. Then we identified alternative synonyms and/or spelling for the major terms from the keywords of related literature, and from the discussion of the authors of this paper. We also split major terms into more specific and clear terms. For example, we split general term non-functional requirements for ML-enabled systems as reliability, usability, explainability, efficiency etc., which we found from \cite{habibullah2021non}, described in \ref{sec:background}. At last we used boolean operators for conjugation, i.e., \textsf{AND} for concatenation of major terms and \textsf{OR} operator to concatenate the alternative synonyms and spelling. 

The search terms are built based on the identified population, intervention, and outcome. \\
\textbf{Population:} Non-functional requirements and their challenges identification process \\
\textbf{Intervention:} Current research and practices in the industry \\
\textbf{Outcomes:} Understanding non-functional requirements and their challenges in machine learning context. \\

The alternative synonyms and spelling for major terms identified are:

\begin{itemize}
    \item \textbf{Machine learning:} (“machine learning" OR “supervised learning" OR “unsupervised learning" OR “reinforcement learning" OR “deep learning")
    
    \item   \textbf{Non-functional requirements:} (“repeatability” OR “reliability” OR "accuracy" OR “reproducibility” OR “consistency” OR “integrity” OR “correctness” OR “fault tolerance” OR “interpretability” OR “transparency” OR “explainability” OR “justifiability” OR “ethics” OR “bias” OR “fairness” OR “performance” OR “efficiency” OR “scalability” OR “domain adaptation” OR “flexibility” OR “adaptability” OR “interoperability” OR “portability” OR “reusability” OR “security” OR “trust” OR “safety” OR “privacy” OR “usability” OR “completeness” OR “maintainability” OR “traceability” OR “testability” OR “retrainability”)
\end{itemize}

We have searched literature in the database for all the non-functional requirements mentioned in \ref{fig:NFRsClusters} using the search string. The following example search terms are used to identify related research papers from database for specified NFRs:
 
 To identify papers on interoperability of ML-ebabled systems we have used \\
 \textbf{(“machine learning" OR “supervised learning" OR “unsupervised learning" OR “reinforcement learning" OR “deep learning") AND ("interoperability")}.
 
To identify usability of ML-ebabled systems we have used \\
 \textbf{(“machine learning" OR “supervised learning" OR “unsupervised learning" OR “reinforcement learning" OR “deep learning") AND ("usability")}.


\subsection{Inclusion and Exclusion Criteria}\label{sec:criteria}

To be useful to answer the research questions, the SLR paper meets the following criteria.

\textbf{Inclusion criteria} \label{inclusionExclusionCriteria}

To be included in the SLR, the paper needs to meet the inclusion criteria.

\begin{itemize}
    \item A paper which focuses on the definition, identification, measurement or challenges of non-functional requirements for machine-learning enabled systems, or different part of the system, e.g., ML model, the data, or the whole system.
    \item A paper which mentions an NFR for machine-learning enabled systems in the list (reliability, usability, explainability, efficiency, flexibility, safety, bias, fairness, transparency, privacy, performance, integrity, security, traceability, ethics, justifiability, data access, completeness, fault tolerance, interpretability, trust, consistency, complexity, data issues, testability, maintainability, retrainability, scalability, portability, reusability, reproducibility, repeatability, interoperability, adaptability, revision, transition). 
    \item Papers which have been published in a peer reviewed journal, conference or workshop.
    \item The articles which are accessible online.
    \item The paper must be written in English.
   
\end{itemize}

\textbf{Exclusion criteria}

\begin{itemize}
    \item Papers that are focused on other topics rather than non-functional requirements for machine learning solutions or systems. This includes papers where an ML approach or algorithm is used to measure, improve, or predict a non-functional requirement or quality of the products or results of ML and not the system or solution itself.
    
    \item Papers which use an NFR as evaluation criteria but do not use the NFR to engineer the system. For example,..................
    
    \item Papers were not written in English.
    \item Papers are not peer reviewed.
    \item Articles whose full text is not available.
\end{itemize}


We created a list of the number of search results for each NFR.  First, we sorted the NFRs in terms of number of papers related to each NFR in decreasing order and excluded those NFRs from our consideration which are extensively covered by other researchers. For example, we have excluded accuracy, efficiency, security, etc., as the number of retrieved papers is relatively high and already well covered by other researchers. 
Then we have filtered out and excluded the non-relevant literature from the rest of the retrieved sources by applying the exclusion criteria mentioned in Section~\ref{inclusionExclusionCriteria}. This process was done by reading the papers' titles, keywords, and abstracts. As a first step, all the authors of this paper read the titles, keywords, and abstracts of the first fifty papers of each NFR individually and filtered the papers. Then we calculated Fleiss' kappa, a statistical measure for assessing inter-coder reliability between a fixed number of raters. Then we arranged several meetings to discuss the papers on which we disagreed. In these meetings, all the researchers read the title and abstract of the article again and finally agreed either to include or exclude the paper after discussion.

 The papers passed in this step were selected for the second stage screening. We checked the number of papers included in this stage after reviewing fifty abstracts of the papers related to each NFR. We decided to exclude those NFRs, which have a high number of included papers after screening fifty papers, as the total included papers will be a large number, which is difficult to include in a single SLR. For example, we found 851 papers from Scopus for Transparency, and after screening 50 papers, we agreed to include 44 papers. Approximately 749 papers will be included for Transparency after screening all the abstracts, which is a very high number for a single NFR; therefore, we excluded Transparency from our consideration.
 
For those NFRs which remained in focus, we read the titles and the abstracts of the second fifty papers related to each NFR to check the consistency of inter-coder reliability and the number of papers we agreed to include. If the inter-coder reliability remains consistent or becomes higher than the previous step, and if the number of papers decided to be included remains low, then we selected those NFRs for the final inclusion in SLR.
 


% Then we discussed together based on our individual filtered results, and included those papers for further investigation which we all agreed those meet the inclusion criteria.


































==> statustable.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\textbf{Section} & \textbf{Last Edited} \\ \hline
Abstract         & Greg                    \\ \hline
Intro            & Greg           \\ \hline
Related Work     & Greg           \\ \hline
Methodology      & Habib            \\ \hline
Results          & Jennifer             \\ \hline
Discussion       &  Habib (not finised yet)                    \\ \hline
Threats          &                      \\ \hline
Conclusions      &                      \\ \hline
\end{tabular}
\end{table}
